Acoustic Identification of Ae. aegypti Mosquitoes using Smartphone Apps and Residual Convolutional Neural Networks

In this paper, we advocate in favor of smartphone apps as low-cost, easy-to-deploy solution for raising awareness among the population on the proliferation of Aedes aegypti mosquitoes. Nevertheless, devising such a smartphone app is challenging, for many reasons, including the required maturity level of techniques for identifying mosquitoes based on features that can be captured using smartphone resources. In this paper, we identify a set of (non-exhaustive) requirements that smartphone apps must meet to become an effective tooling in the fight against Ae. aegypti, and advance the state-of-the-art with (i) a residual convolutional neural network for classifying Ae. aegypti mosquitoes from their wingbeat sound, (ii) a methodology for reducing the influence of background noise in the classification process, and (iii) a dataset for benchmarking solutions for detecting Ae. aegypti mosquitoes from wingbeat sound recordings. From the analysis of accuracy and recall, we provide evidence that convolutional neural networks have potential as a cornerstone for tracking mosquito apps for smartphones.

==> attic/03_methodology_BACKUP.tex <==
\section{Materials and Methods}
\label{sec:methodology}
 

\subsection{Data Collection} 
\label{sec:methodology:data}

\begin{itemize}
    \item \red{Falar sobre os conjuntos de gravações que serão usados no escopo do presente trabalho.}
    \item 1190 gravações de mosquitos com variadas: quantidade mosquitos, espécie de mosquitos	sexo mosquitos, idade de mosquitos e	método de coleta. 
    \item ??? gravações de ambiente sem mosquitos.
    \item \red{Consultar a Tabela~\ref{tab:datasets}.}
\end{itemize}

 
\begin{table}[htb]
    \centering
    \begin{tabular}{c l}
    \textbf{ID} & \textbf{Description} \\ 
     DT1 &	Somente gravações de Ae. aegypti macho + gravações sem mosquitos	\\						
DT2	& Somente gravações de Ae. aegypti fêmea + gravações sem mosquitos		\\					
DT3	& Somente gravações de Ae. aegypti macho e fêmea + gravações sem mosquitos	\\						
DT4	&  Ae. aegypti macho e fêmea + gravações de Ae. albopictus + gravações de outros mosquitos + gravações sem mosquitos							\\
    \end{tabular}
    \caption{Conjuntos de gravações disponíveis para os experimentos com distribuição uniforme.}
    \label{tab:datasets}
\end{table}

% \subsection{Capture processing} 

% \begin{itemize}
% \item Capacidade de captura dispositivos
% \item Eficiência da captura contínua
% \end{itemize}

\subsection{Audio Pre-processing}
\label{sec:methodology:pre-processing}

\begin{itemize}
    \item \red{Sobre o impacto da deterioração das gravações de mosquitos:}
\begin{itemize}
\item \red{Attenuation Normalization: ocorre atenuação devido a variação na distância entre mosquito e microfone. Abordagem proposta é normalizar audio.}
\item \red{Distortion Reduction: ocorre distorção de fase devido a sobreposição de ondas refletidas. Assumir que o impacto é irrelevante (impacto do microfone?) e deixar para trabalhos futuros (TODO: posição do UNet-wave sobre isso?.}
\item \red{Noise Filtering: sobreposição de frequências de outras fontes (outros mosquitos e ambiente). Abordagem proposta é usar UNet-wave (TODO: olhar o artigo ve se autores abordam os outros tipos de problemas).}
\item \red{Ver Figura~\ref{fig:audio_clips}.}
\end{itemize}
\end{itemize}

\begin{figure}[htb]
\centerline{
    \subfigure[beginning audio clip - before processing]{\includegraphics[width=.3\textwidth]{example-image-c}
    \label{fig:sens_topologia}} 
        \hfil
    \subfigure[beginning audio clip -  after processing]{\includegraphics[width=.3\textwidth]{example-image-c} \label{fig:sens_limiar}} 
        \hfil
    \subfigure[beginning audio clip - ground truth processing]{\includegraphics[width=.3\textwidth]{example-image-c} \label{fig:sens_limiar}} 
} 
\centerline{
    \subfigure[middle audio clip - before processing]{\includegraphics[width=.3\textwidth]{example-image-c}
    \label{fig:sens_topologia}} 
        \hfil
    \subfigure[middle audio clip -  after processing]{\includegraphics[width=.3\textwidth]{example-image-c} \label{fig:sens_limiar}} 
        \hfil
    \subfigure[middle audio clip - ground truth processing]{\includegraphics[width=.3\textwidth]{example-image-c} \label{fig:sens_limiar}} 
} 
\centerline{
    \subfigure[ending audio clip - before processing]{\includegraphics[width=.3\textwidth]{example-image-c}
    \label{fig:sens_topologia}} 
        \hfil
    \subfigure[ending audio clip -  after processing]{\includegraphics[width=.3\textwidth]{example-image-c} \label{fig:sens_limiar}} 
        \hfil
    \subfigure[ending audio clip - ground truth processing]{\includegraphics[width=.3\textwidth]{example-image-c} \label{fig:sens_limiar}} 
} 
   \caption{Audio clips}
   \label{fig:audio_clips}
\end{figure} %TODO: gerar figuras e colocar no repositório do artigo e colocar link do repositório aqui.

\subsection{Features Extraction}
\label{sec:methodology:features}

\begin{itemize}
\item \red{Apresentar a Transformada de Fourier.}
\item \red{Apresentar a Escala Mel (see Figure~\ref{fig:audio_mel}).}
\item \red{Discutir sobre a escolha de parâmetros da transformada e da escala para extração de features.}
\end{itemize}

\begin{figure}
    \centering
    \includegraphics[width=.3\textwidth]{example-image-b}
    \caption{Exemplo de amostra em escala Mel}
    \label{fig:audio_mel}
\end{figure}
 
\subsection{Neural Networks}
\label{sec:methodology:neural}

\begin{itemize}
    \item \red{Apresentar a eede baseada em Unet-Wave para enaltecimento de gravações.}
    \item \red{Apresentar a rede convolutiva específica para classificação composta por:}
    \begin{itemize}
        \item \red{Conjunto de Bloco identificadores oferecem flexibilidade visando efácia e eficiência em cada domínio alvo (e.g. incidência de certos mosquitos e ruídos na região alvo).}
        \item \red{Bloco Cluster permite maior eficácia de classificação em comparação com ranqueamento simples.}
    \end{itemize}
\end{itemize}

\subsection{Model Evaluation}
\label{sec:methodology:model}

\red{Em resumo, a ideia é apresentar a mesma argumentação do artigo anterior \citep{FERNANDES2021104152}. No caso, vislumbra-se adicionar novas métricas de verificação da eficácia da proposta, incluindo de enaltecimento de audio.}

\red{Abaixo segue uma relação de possíveis métricas a serem consideradas no estudo:}
\begin{itemize}
    \item \red{Accuracy.} 
    \item \red{Precision.}
    \item \red{Recall.}
    \item \red{F1-measure.}
    \item \red{Especificidade (?).}
    \item \red{Métricas de audio (?) (TODO: ver as métricas usadas na Unet-Wave).}
\end{itemize}


%RM: esta seção distribuí em outras
% 4.3 Classification processing: (0,5 página):
% Extração de features
% Normalização de áudio
% Processo de classificação
% Flexibilidade

%RM: acho que isso fica de fora neste trabalho
% 4.4 Hardware restriction: (0,5 página):
% Carga computacional
% Dispositivos móveis
% Dispositivos IoT

==> attic/04_proposal_BACKUP.tex <==
\section{Proposed Approach} %Mariana
\label{sec:proposal}
%RM: implementação?

\begin{figure}
    \centering
    \includegraphics[width=.5\textwidth]{example-image-a}
    \caption{Processo de captura não linear -> Pré-Processamento de áudio -> Extração de features -> Classificação}
    \label{fig:my_label}
\end{figure}
 
 
% \subsection{Capture audio}
% %RM: acho que isso é sobre o APP e acho que não entraria neste paper
% \begin{itemize}
%     \item Processo de captura não linear
%     \item Otimização computacional
%     \item Simultaneidade de captura e classificação 
% \end{itemize}


\subsection{Enaltencimento de Audio}
\label{sec:proposal:pre-processing}

\begin{itemize}
    \item \red{Discutir a normalização de atenuação usando escala Mel e transformada de Fourier parametrizados.}
   % \item Otimização computacional (Distortion Reduction)
    \item \red{Apresentar a técnica de filtragem de ruídos (que será extremamente útil para a operação da rede com gravações feita em ambiente não controlado) usando UnetWave.}
\end{itemize}
 
 
\subsection{Audio Classification}
\label{sec:proposal:classification}

\begin{itemize}
    \item \red{Apresentar a rede convolutiva específica para classificação de gravações do mosquito, composta por:}
    \begin{itemize}
        \item \red{Conjunto de Bloco identificadores oferecem flexibilidade visando efácia e eficiência em cada domínio alvo (e.g. incidência de certos mosquitos e ruídos na região alvo).}
        \item \red{Bloco Cluster permite maior eficácia de classificação em comparação com ranqueamento simples.}
    \end{itemize}

\end{itemize}

\begin{figure}
    \centering
    \includegraphics[width=.5\textwidth]{example-image-b}
    \caption{NN architecture overview.}
    \label{fig:my_label}
\end{figure}

 
\begin{figure}[htb]
\centerline{
    \subfigure[Identification Block]{\includegraphics[width=.3\textwidth]{example-image-c}
    \label{fig:sens_topologia}} 
     \hfil
\subfigure[Cluster Block]{\includegraphics[width=.3\textwidth]{example-image-c} \label{fig:sens_limiar}} 
   } 
   \caption{NN architecture main building blocks}
   \label{fig:sensibilidade}
\end{figure} 

==> attic/05_evaluation_BACKUP.tex <==
\section{Experiments and Results}
\label{sec:evaluation}

\subsection{Análise de Eficácia e Eficiência Comparada com o Trabalho Anterior}
\label{sec:evaluation:efficiency}

\red{A ideia é apresentar aqui os resultados obtidos com a nova rede neural, comparando com os resultados obtidos com a versão do trabalho anterior \citep{FERNANDES2021104152}, considerando o conjunto de gravações D1 (conforme Tabela~\ref{tab:datasets}):}
\begin{itemize}
 \item \red{Apresentar os resultados da nova rede neural e a do trabalho anterior \citep{FERNANDES2021104152}}
 \item \red{Analisar a eficácia da nova rede neural em comparação com a do trabalho anterior em termos de acurácia, precisão, recall e F1-score}
 \item \red{Analisar a eficiência da nova rede neural em comparação com a do trabalho anterior em termos de tamanho e complexidade da rede neural}
\end{itemize}

\subsection{Análise da Efetividade da Nova Rede Neural em Gravações com Ruído Artificial}
\label{sec:evaluation:noise}
\red{Usando o conjunto de gravações D4, que corresponde ao conjunto de gravações D2 com ruído adicionado artificialmente, seguindo metodologia UnetWave:}
\begin{itemize}
 \item \red{Analisar os resultados da nova rede neural usando pré-processamento, e comparar com a rede neural do trabalho anterior \citep{FERNANDES2021104152}}
 \item \red{Apresentar os resultados de classificação da nova rede neural treinada com o conjunto de gravações D4}
 \item \red{Apresentar os resultados de classificação da nova rede neural treinada com o conjunto de gravações D4 pré-processado}
\end{itemize}
 
\subsection{Análise da Efetividade da Nova Rede Neural em Gravações com Ruído Natural}
\label{sec:evaluation:efficiency}

\red{Nesta seção, serão apresentados os resultados com gravações que contém ruídos ambientes, gravados junto com os mosquitos. Nesse caso, deverá ser usado o conjunto de gravações D3, que possui ruído natural.}

\begin{itemize}
 \item \red{Analisar os resultados da nova rede neural com gravação ruidosa}
 \item \red{Apresentar os resultados de classificação da nova rede neural treinada com o conjunto de gravações D3}
\end{itemize}


% \subsection{Generalizing the Classification Process}
% \label{sec:evaluation:efficiency}

% \begin{itemize}
% \item \red{Usando D2}
%  \item \red{RNAv2 apresenta resultados equivalentes treinando e classificando com datasets distintos.}
%  \item \red{Treina RNAv2 com D2 e classifica D2}
%  \item \red{Treina RNAv2 com D1 e classifica D2}
% \end{itemize}



==> attic/revision-letter-R1.tex <==
\begin{coverletter}

\noindent \Large Revision Letter

\vspace{0.3cm}

\noindent \large \textbf{Detecting \aedes Mosquitoes through Audio Classification with Convolutional Neural Networks}

\vspace{0.2cm}

\noindent \normalsize Marcelo Schreiber Fernandes,Weverton Cordeiro,Mariana Recamonde-Mendoza \\

\noindent \textbf{Principal Corresponding Author and E-mail:} Mariana Recamonde-Mendoza (mrmendoza@inf.ufrgs.br) \\

\noindent \textbf{Contact Address:} Institute of Informatics -- Federal University of Rio Grande do Sul (UFRGS), Av. Bento Gon\c{c}alves, 9500, Agronomia, 90.501-970, Porto Alegre, Brazil. \textbf{Phone:} +55 51 3308-6843 \textbf{Fax:} +55 (51) 3308-7308 \\

\vspace{0.9cm}

\noindent Dear Dr. \textbf{Edward Ciaccio} (Editor-in-Chief, Computers in Biology and Medicine),
\\
\\
Please find attached a revised version of our manuscript we submit to the Elsevier Computers in Biology and Medicine Journal. We worked hard to address each of the reviewers' comments and suggestions since we received the initial decision and revised our manuscript to accommodate them to the best of our efforts.\\
\\
In summary, we performed the following major changes and improvements to our manuscript:

\begin{itemize}
  \item We provided further detail on the previous work that also used the same mosquito wingbeat recording dataset that supported our research and complemented the description of the downloaded dataset to clarify aspects regarding acoustic data collection (types of mobile phones used in the recording, background noise, etc.);
  \item We improved the discussion of the data augmentation strategy we use to generate more recordings for training and compensate for the limited set of wingbeat recordings we used in our research;
  \item We provided a more detailed view of the deep architectures deployed in our experiments, as well as other features like the size of input audio segments, dimensions of the spectrogram fed as input to the neural network, etc.;
  \item We carried out further experiments to observe the change in performance for the whole ensemble upon the removal of a classifier that presented the worst class imbalance in our ensemble observing, as a result, a little to marginal impact to overall performance;
  \item We retrained our binary classification model using the average-pooling function in place of the max-pooling function and verified that the max-pooling results are superior to the results with average-pooling.
\end{itemize}
\\
In the revised manuscript, we also (i) clarified that we used the only publicly available dataset of mosquito recordings to support our work, (ii) discussed the issue of class imbalance and how it had little to marginal effect to our results, (iii) provided more information about the data recording in the experimental dataset and clarified the importance of the characteristics of the dataset recordings, and (iv) clarified other aspects like kernel sizes considered, loss function used, cross-validation, use of cross-entropy loss for model training and macro-average for performance measurement, and major voting strategy. The letter to reviewers provides a detailed list of considerations to the reviewers' comments and changes made in the manuscript.\\
\\
We want to thank the editor and the reviewers for their valuable feedback on our research and manuscript. Having reflected upon their comments and suggestions and accommodated them in our submission, we firmly believe that we came up with a more robust version of our manuscript, as discussed in the point-by-point response to the reviewers.\\
\\
Yours sincerely,\\
\\
The authors.
\end{coverletter}

==> attic/revision-letter-R2.tex <==
\begin{coverletter}

\noindent \Large Revision Letter

\vspace{0.3cm}

\noindent \large \textbf{Detecting \aedes Mosquitoes through Audio Classification with Convolutional Neural Networks}

\vspace{0.2cm}

\noindent \normalsize Marcelo Schreiber Fernandes,Weverton Cordeiro,Mariana Recamonde-Mendoza \\

\noindent \textbf{Principal Corresponding Author and E-mail:} Mariana Recamonde-Mendoza (mrmendoza@inf.ufrgs.br) \\

\noindent \textbf{Contact Address:} Institute of Informatics -- Federal University of Rio Grande do Sul (UFRGS), Av. Bento Gon\c{c}alves, 9500, Agronomia, 90.501-970, Porto Alegre, Brazil. \textbf{Phone:} +55 51 3308-6843 \textbf{Fax:} +55 (51) 3308-7308 \\

\vspace{0.9cm}

\noindent Dear Dr. \textbf{Edward Ciaccio} (Editor-in-Chief, Computers in Biology and Medicine),
\\
\\
Please find attached the second revised version of our manuscript we submit to the Elsevier Computers in Biology and Medicine Journal. In summary, we performed the following modifications to the manuscript:\\

\begin{itemize}
    % Reviewer Comment:  1. The input dimensions of the deep architectures. 
    
    \item We clarified the input dimensions of the deep architectures, as requested by the reviewer. To this end, we modified Figure 2, Figure 4, as well as the description of the data pre-processing (Section 3.1) and feature extraction (Section 3.2), the proposed approach (Section 4), and part of the experimental evaluation (Section 5.1). More specifically, we emphasized the dimensions of the output array of the FFT function for a given sample, and which is used as input for training each of the CNN models (binary classifier, multiclass classifier, and ensemble of binary classifiers). In particular, we emphasized in Section 3.2 and Section 4 that the input of the model training is an array with dimensions m x n x 1, where m equals the number of bands and n equals the number of frames used as parameters in the FFT. Then in Section 5.1 we discussed the assessment of the performance obtained with various parameter settings for the number of bands and frames, and emphasized the choice in our training of an input having dimensions 60 bands x 40 frames x 1.
    
    % Reviewer Comment: 2. The reasons of choosing current deep architectures, such as the different 20x5 and 8x4 kernels, should be explained in the paper.

    \item We discussed the reasons of choosing current deep architectures, such as the different 20x5 and 8x4 kernels, in response to the reviewer's comment. To this end, we included a novel section to discuss architectural settings for classifiers (Section 4.4). In that section, we discussed the choice of the CNN architectures, including the rationale for adjusting the network architecture according to the type of classification problem. It includes the discussion of the results that led us to the use of 20 x 5 and 8 x 4 kernels in our multiclass classifier, for example. We also discussed in this section the literature review carried out to support our choice for parameters and settings for input dimensons, kernel size and shape, and use of max-pooling and average-pooling.
\end{itemize}

\vspace{1.5cm}

\noindent Yours sincerely,\\
\\
\\
The authors.
\end{coverletter}
